Robotics Software Engineering: A Perspective from the Service Robotics Domain

Robots that support humans by performing useful tasks (a.k.a., service robots) are booming worldwide. In contrast to industrial robots, the development of service robots comes with severe software engineering challenges, since they require high levels of robustness and autonomy to operate in highly heterogeneous environments. As a domain with critical safety implications, service robotics faces a need for sound software development practices. In this paper, we present the first large-scale empirical study to assess the state of the art and practice of robotics software engineering. We conducted 18 semi-structured interviews with industrial practitioners working in 15 companies from 9 different countries and a survey with 156 respondents (from 26 countries) from the robotics domain. Our results provide a comprehensive picture of (i) the practices applied by robotics industrial and academic practitioners, including processes, paradigms, languages, tools, frameworks, and reuse practices, (ii) the distinguishing characteristics of robotics software engineering, and (iii) recurrent challenges usually faced, together with adopted solutions. The paper concludes by discussing observations, derived hypotheses, and proposed actions for researchers and practitioners.

==> Sections/conclusion.tex <==
\section{Conclusion and Recommendations}
\label{sec:conclusion}
In this paper, we presented an empirical assessment of the current state of robotics software engineering. 
The study comprehends 18 interviews with industrial practitioners from 15 different companies and a survey with 156 respondents from the robotics domain.

The collected data allowed us to answer the three research questions formulated in the introduction and to recommend some research themes that deserve further investigation.

%\begin{itemize}[leftmargin=5.5mm]
	%\item {\bf Testing}.
	\parhead{Testing}
	Our results point out the paramount role of robustness and validation.
	 They emphasize the importance of real-world testing, since simulations are not precise enough to support the discovery of problematic situations.
	However, as real-world testing is expensive, practitioners would largely benefit from techniques that provide realistic test data.
	Most contemporary methods in the testing domain generate test data by relying on code-centric information like coverage criteria and input spaces.
	In contrast, there is a potential for novel testing techniques that consider historical real-world data and use them for systematically producing new critical scenarios.

	%\item {\bf Standardized solutions}. 
	\looseness=-1
	\parhead{Standardized Solutions}
	The development of  robotic software mostly consists in integrating reusable components that implement recurrent functionalities. % according to the specific requirements of each specific application. 
	While de-facto standards at the level of hardware interfaces and inter-component communication (e.g., ROS messages) exist, reference models that capture reusable solutions for recurrent problems in applications development are still missing. 
	The OMG Robotics Domain Task Force~\cite{omg-robotics} aims at fostering the integration of robotic systems from modular components through the adoption of OMG standards. 
	To the best of our knowledge,  it does not seem to have produced relevant results so far.

%	\item {\bf AI and ML}. 
\looseness=-1
	\parhead{AI and ML}
	Surprisingly, our study does not identify AI and  ML as prevalent technologies in the robotic domain. 
	Most survey respondents' organizations do not use AI techniques and they do not foreseen the use of AI and ML as a big challenge. This might be interpreted in various ways. 
	It seems that those using AI and ML (e.g.,  for computer vision), feel that the libraries that are readily available are trusted. %and of good quality. 
	On the other side, we might interpret this result considering that most of the available robotic solutions   are tailored to a specific task and/or are able to work in a controllable and known environment. 
	Probably, in the near future, when robots will be required to work under uncertainty in uncontrollable and unknown environments, interest in AI and ML will grow in the community. 
	This was advocated by works as the one by Ingrand et al.~\cite{ingrand2014robotics}, which provides several contributions that addressed deliberation
	from the AI–Robotics point of view.

%	\item {\bf Academia vs Industry}. 
	\parhead{Academia vs Industry}
	We identify a gap between the solutions provided by the research community (e.g. the variety of robotics middleware, component frameworks, model-driven environments, software engineering processes and methodologies) and the current practice in robotics industry (mostly focused on code implementation and integration mismatch resolution). 
	This could be due to the nature of current research in software engineering for robotics, which lacks of an overall vision of the current needs in industrial practice and has produced fragmented solutions.
%\end{itemize}

%We report the practices applied by the participants to the study, who are mainly focused on the software implementation, using mostly object-orienting programming and CBSE.
%...
%Finally, based on our findings from this study, we provide a synthesized list of opportunities for the robotics software engineering community.

%\ds{Commented out the following part -- if we end with big themes for future research, I think it's not necessary to expand on future work in the narrower sense.}
%
%As future work, we plan to extend our work by:
%\begin{enumerate*}
	%\item investigating reuse styles, how much is actually used copy-paste-modify with respect to systematic approaches;
	%%\item identifying most common ways of ensuring the interoperability of heterogeneous components in robotic applications;
	%\item studying the impact and necessity of mission specification for teams of robots;
	%\item further researching challenges identified by respondents.
%\end{enumerate*}

==> Sections/discussion.tex <==
\section{Discussion}
\label{sec:discussion}

==> Sections/mission.tex <==
\section{Perception of Robotics Software Engineering (RQ2)}
\label{sec:rq2}
RQ2 details distinguishing characteristics of robotics software engineering and how it differs from other domains, in particular from other cyber-physical sub-domains.
In particular, we describe \sergio{differs open-ended question}, who specifies missions for robots and what methods they use. 

\begin{figure}[htb]
	\begin{center}
		\includegraphics[trim=0.5cm 0cm 0cm 0cm, clip=true, width=\columnwidth]{../material/survey/script/graphs/all/likert/mission_filtered.pdf}
		\smash{\begin{minipage}{8.5cm}
				\begin{scriptsize}
					\leftline{``Don't know'' (from top to bottom):}
					\leftline{24\%, 77\%, 37\%, 17\%, 40\%} 
				\end{scriptsize}
				\vspace{1.5cm}
		\end{minipage}}
		\vspace{-1.2cm}
		\caption{
			Mission specification methods (all roles).
			%``I don't know'' response's rate, ordered: 24\%, 77\%, 37\%, 17\%,   and 40\%.
		}
		\label{fig:specify} 
		\vspace{0.2cm}
	\end{center}
\end{figure}

\parhead{Mission specification}
Fig.~\ref{fig:specify} shows the most used mission specification methods according to our survey's results.
The most common way for specifying missions is to hard-code them, 56\% of the participants always or very often use this method.
They survey permitted participants to answer in an open-ended text an alternative method after responding ``Other'' (29\%).
The collected answers refer to methods as Behavior Trees~\cite{BTs}, State Machines, and configuration files.
However, the most repeated method are Graphical User Interfaces (4 out of 15 answers, 26.7\%).
The third most common method are self-developed DSLs (27\%), being a difference between practitioners (34\%) and academics (16\%).
The least common options are using logical languages (e.g., LTL) with 6\% and using third-party DSLs (5\%).
The  ``I don't know'' answer's rates are: 24\%, 77\%, 37\%, 17\%, and 40\% for hard-coded, other, self-developed DSLs, logical language, and third-party DSLs, respectively.
Table~\ref{tab:mission} summarizes the survey's results of which stakeholders typically are in charge of specifying missions for robots.
Most of the overall of participants chose developers (55.8\%).
The second place is for  technically skilled end-users  (55.2\%) and the third for non-technically skilled end-users (44.2\%).
The least common stakeholder is integrators, with 23.4\%.
Contrary to practitioners, the results for academics show a wide gap developers (67.9\%) and non-technical end-users (30.4\%).

\vspace{0.4cm}
\input{tables/mission.tex}

The ``I don't know'' rate implies confusion from the participants' side with respect to mission specification methods.
Intrigued, we dug deep for more details in the interviews, and realized that some interviewees were not familiar with the term ``mission specification'', what required some explanation from us.
Most of them perform and provide tools for mission specification.
Those tools include GUIs (almost half of the cases), DSLs, or hard-coded solutions.


The fact that hard-coding is the most common mission specification method (56\%),  implies a reduced usability and flexibility of nowadays robotic systems.
This percentage may seem contradictory taking into account that most commonly end-users specify the robotic missions.
However, these end-users are technically-skilled, so they possess the knowledge to encode a mission using, for instance, a programming language as Python.
Another method, which was pointed by participants are GUIs---which in fact can be considered DSLs---provides certain flexibility to the user for mission specification. %for such specification to, for example, allow users to specify the waypoints to be reached by the used robots.
Fig.~\ref{fig:languages} and Fig.~\ref{fig:specify} corroborate that the usage of DSLs is currently limited in robotics.
Nevertheless, we observed that practitioners make use more often of DSLs  (34\%) than academics  (16\%) for mission specification.
There is also a significant difference between the usage of home-grown DSLs and third-party DSLs (27\% and 5\%, respectively) across all the roles.
We argue its relation to the roadblocks to reused discussed in Section~\ref{sec:rq1}.
Practitioners do use more commonly GUI-based approaches and DSLs than academics, but both roles end-up using hard-coded solutions the same (54\% and 57\%, respectively.).
Factory automation (the most common application field according to the results showed in Section~\ref{sec:context}), mobile robots are pre-programmed to perform a automated missions (e.g., moving from A to B). 
The destination is generated automatically by a SCADA system or an Enterprise Management System. 
An example of systems that integrate such pre-programmed mobile robot mobile are the ones used in Amazon Warehouses. 
Those robots move along routes that are generated according to what customers have ordered through the online portal.
To what it concerns with industrial arms, they are programmed to perform specific tasks by an expert using a robot-specific programming language.

The most common stakeholder for mission specification are developers (55.8\%), which may mean that the participants:
\begin{enumerate*}
	\item do not provide a complete robotic system, so they are in charge of specifying missions the their own robots;
	\item provide a complete robotic system and pre-defines a (set of) missions for it; or
	\item provide a complete robotic system and the typical client is another developer.
\end{enumerate*}
According to the practitioners' results, the percentage's differences between stakeholders are minimal.
Oppositely, academics rarely rely on end-users (especially non-technical ones, with 30.4\%) to specify missions for robots.






==> Sections/opportunities.tex <==

%\section{Identified Research Directions}\label{sec:opportunities}
%\chg{Based on the findings from our study, we propose a suite of opportunities for practitioners and the robotics software engineering community in general.
%We have identified during this study the importance of testing for the robotics software engineering community.}{During this study we identified some important research directions for practitioners and the robotics software engineering community in general.}
%
%
%\ins{\noindent {\bf Runtime V\&V.}}
%Due to the intrinsic  characteristics of robotic systems defined in Section~\ref{sec:rq2}, testing should be tailored to running systems, which are executed in the actual environment.
%Nowadays, there are no established automatized testing processes for run-time systems which also involve hardware.
%Runtime verification is \ugh{an analysis and execution approach that provides a formal manner of runtime testing  cyber-physical systems as robots.}
%It has been already implemented on robotic~\cite{huang2014rosrv}   and component-based~\cite{falcone2011runtime}   systems and could be integrated with existing monitoring tools~\cite{rviz}.
%
%
%Also, we learned that roboticists perform real-world experiments almost as often as simulation.
%The cause is most roboticists do not ``trust'' simulated tests and strive to start experiment in real-world situations as soon as feasible.
%However, testing  real-world scenarios often becomes a time-consuming and error-prone process due to  experiment planning flaws.
%Also, this often limit the scope of an application to the context and robotic platform where it can be tested.
%This causes that reused algorithms often need severe adjustments to work reasonably in other use cases.
%Therefore, existing simulation tools and frameworks must improve to ease this problem and shorten the gap between simulation and real-world experimentation.
%Promising techniques as machine and reinforcement learning---which have been already applied enhance object recognition and collision avoidance in robotics---may be put to use for this topic.
%Following the same idea, these techniques are very promising for allowing robotic applications to deal with uncertainty and partial knowledge in the environment~\cite{bozhinoski2019safety}.
%However, the use of machine learning for safety critical systems is still open~\cite{mallozzi2018keeping}.
%
%\ins{\noindent {\bf Standards and certification}.} Another recurrent challenge we documented in this work is the current lack of standards in the community.
%This hinders  robotic development and complicates software reuse.
%The ROS Industrial project~\cite{ros-industrial}  works to solve this problem by creating and using  standardized ROS messages as interfaces to stimulate ``hardware-agnostic'' software development.
%However,  it does not seem to be adequate to solve these problems because its activities mostly aim at defining standards at the level of hardware interface to industrial products and not at the system and application levels.
%\ugh{To tackle this challenge, we propose the adopt methodologies, best practices, and standards that have demonstrated their usefulness from other industrial domains} (A-SPICE~\cite{AutomotiveSIG2015}, ISO9000).
%
%
%\ins{\noindent {\bf Systematic approaches to software development}.} Various projects have promoted the adoption of systematic approaches to software development and integration in robotics: NASA JPL Claraty~\cite{volpe2001claraty}, EU FP7 BRICS~\cite{bischoff2010brics}, H2020 RobMosys~\cite{euh2020}, RoboCup~\cite{kitano1995robocup} challenges. 
%We see a lack of involvement of the SE community in these projects, lack of interest of the industry in this kind of research activities, and limited technology transfer. 
%Our envisioned solution involves the development of  a software foundation, like Eclipse, Apache, or the Linux Foundation, specifically focused on Robotic Software Engineering. 
%The main purpose of the existing OMG Robotics Domain Task Force~\cite{omg-robotics}  is to foster the integration of robotics systems from modular components through the adoption of OMG standards.
%To the best of our knowledge,  it does not seem to have produced relevant results so far. 
%
%\subsection{others}
%
%One response states that the community should collect and develop specific design patterns for robotics.
%\begin{itemize}
%	\item Design Patterns for Behavior-Based Robotics
%	\item https://corlab.github.io/dslzoo/design-patterns-discipline.html
%\end{itemize}
%
%
%Modeling
%
%RE?
%
%%In this section we describe opportunities to close the gap between robotics SE challenges.
%%For this, we analyze data from a survey's open-ended question where we requested respondents to answer how current robotics  SE practices should change.
%%As previously done, we coded the total of 79 answers to the questions, and coded 90 textual responses out of them.
%%Opposed to the majority, 5 respondents do not see a need in changing the current practices in robotics SE.
%%5 more respondents where not sure, had no strong opinion, or were not sure whether there are any practices at all.
%%
%%Almost half of the responses (41) asks for a general shift of the community to improve the current software development practices in robotics.
%%13 respondents explicitly ask for a shift of the community towards general SE approaches.
%%In particular, they argue about the promotion of modular and reusable code, favor parametrization to hard-coding, proper code style and design, etc.
%%Among the total, 7 responses claim that there is a need of increasing the resusability of software, not only in terms of software and frameworks, but also \textit{across robots}.
%%As one of the respondents pointed, the usage of common and widely established functional libraries (as OpenCV in Computer Vision~\cite{opencv_library}) could mitigate such problems.
%%4 responses  request the streamline of effort towards modularity in software development, a SE best practices that enhances software reusability.
%%According to 16 responses,  to reach a more systematic, formal and better quality manner of developing, analyzing, and verifying robotic applications, practitioners must adhere to modeling practices.
%%2 responses state that is needed to reach a better understanding of software architectures so to enhance a more structured development of reliable software.
%%Other responses (3) state that roboticists should take advantage of methodologies and techniques which reliability has been proved in other industry domains for software development.
%%One response states that the community should collect and develop specific design patterns for robotics.
%%Another petition from two respondents is the need of performing further analysis of data of current established knowledge, which should be then surveyed and systematized.
%%This is our main goal with this work.
%%
%%14 respondents stress the impact of lack of standards to which the robotics community can adhere.
%%As we have discussed previously in this paper %(see Section~\ref{subsec:paradigms}, Section~\ref{subsec:lang}, Section~\ref{subsec:qa}, Section~\ref{sec:rq2}, and  this section)
%%robotic practitioners are mostly focused  on the implementation of small pieces (i.e., components) of the overall puzzle that characterizes robot control applications.
%%2 respondents  expect to lower the effort needed to integrate components, allowing developers to focus on the logic side of the code by enforcing standards.
%%We count 3 respondents that call for a firmer community-wide commitment to create and maintain open-source references and standards to stop practitioners from ``reinventing the wheel.''
%%\qsxperroni{ROS distributions are a start, but are still far from ideal.}
%%
%%\looseness=-1
%%A substantial number of respondents (9)  think that what should change in  robotics SE is the mindset of the community.
%%The majority of these claims 6 request more usage of the Open Source world, requesting explicitly to industry a bigger ``openness''.
%%2 other arguments   ask to industry for a more progressive mindset with respect to know technologies, such as AI to permit the evolution of the software development processes in robotics.
%%There are also comments (2) which request a more ``enterprise-grade'' software engineering instead the research-style in which robotics mainly works nowadays and to aim to solve real-world problems instead of  not existing ones.
%%
%%The rest of the responses mostly ask for a better suite of tools and frameworks to improve the support of \textit{automated and systematic} testing of linked software and hardware and realistic simulation.
%
%


==> Sections/related.tex <==
\section{Related Work}



==> Sections/results.tex <==










==> tables/companies.tex <==
%\item 
%\item 
%\item 
%\item 
%\item 

\begin{table}[h!]
	\caption{Companies involved in our multiple-case study}
	\vspace{-0.3cm}
	\label{tab:companies}
	\small
	\begin{tabular}{ p{0.05cm}  p{7.8cm}  } %{ l  c c c  c }
		\toprule
		\hspace{-0.2cm}\parbox[t]{0.2cm}{\textsf{A}}	
		&
		A small-sized company specialized in outdoor mobile robots and professional Research and Development (R\&D) consultancy.
		\\
	%	\midrule
		
		\hspace{-0.2cm}\parbox[t]{0.2cm}{\textsf{B}}
		&
		A small-sized company, which focuses on autonomous navigation solutions.
		 \\
%		\midrule
		
		\hspace{-0.2cm}\parbox[t]{0.2cm}{\textsf{C}}
		&
		A large-sized company that mainly works in the field of engineering and electronics and that is currently investing in Artificial Intelligence (AI) and robotics.	
		 \\

		\hspace{-0.2cm}\parbox[t]{0.2cm}{\textsf{D}}
		&
		A large-sized technological center working mainly in applied R\&D.
		 \\

		\hspace{-0.2cm}\parbox[t]{0.2cm}{\textsf{E}}
		&
		a small-sized company that manufactures humanoid robots and research robotic platforms. 
		\\
		
		\hspace{-0.2cm}\parbox[t]{0.2cm}{\textsf{F}}
		&
		A small-sized company that develops and manufactures mobile service robotic platforms. 
		\\
		
		\hspace{-0.2cm}\parbox[t]{0.2cm}{\textsf{G}}
		&
		A large-sized company working in the intralogistics sector.
		\\
		
		\hspace{-0.2cm}\parbox[t]{0.2cm}{\textsf{H}}
		&
		A technology-oriented large-sized company, which also invests in robotics. 
		\\
		
		\hspace{-0.2cm}\parbox[t]{0.2cm}{\textsf{I}}
		&
		A large-sized technology institute, which focuses in diverse industrial fields, including mobile robots.
		\\
		
		\hspace{-0.2cm}\parbox[t]{0.2cm}{\textsf{J}}
		&
		 A medium-sized company that provides self-driving products and services.
		\\
		
		\hspace{-0.2cm}\parbox[t]{0.2cm}{\textsf{K}}
		&
		a micro-business which develops and rents customer-tailored robotic solutions.
		\\
		
		\hspace{-0.2cm}\parbox[t]{0.2cm}{\textsf{L}}
		&
		A micro-enterprise with the aim of developing and renting modular robot-based solutions.
		\\
		
		\hspace{-0.2cm}\parbox[t]{0.2cm}{\textsf{M}}
		&
		A large-scale company mainly working in the aviation sector, and which also works with unmanned air vehicles.
		\\
		
		\hspace{-0.2cm}\parbox[t]{0.2cm}{\textsf{N}}
		&
		A large-sized research institute with focus on industrial projects, including artificial intelligence in automation.
		\\
		
		\hspace{-0.2cm}\parbox[t]{0.2cm}{\textsf{O}}
		&
		A small-sized company, which specializes in educational technology by means of service robots.
		\\

		\bottomrule
	\end{tabular}
\end{table}


==> tables/mission.tex <==

\begin{table}[h!]
	\caption{Stakeholders who specify robotic missions}
	\vspace{-0.2cm}
	\label{tab:mission}
	\small
	\begin{tabular}{ p{1cm}  P{1.05cm}   P{0.95cm} P{1.65cm} P{1cm}  P{0.5cm}} %{ l  c c c  c }
		\toprule
		& &\multicolumn{2}{c }{\textsf{End-users}} &&\\
		\cline{3-4}  
		&  \textsf{Developer} & \textsf{Technical} & \textsf{Non-technical}  & \textsf{Integrator} & \textsf{Other}\\
		\midrule 
		\hspace{-0.2cm}\parbox[t]{1cm}{ \textsf{Overall}}	
		%textsf{Overall}
		&
		55.8\,\%
		&
		55.2\,\%
		&
		44.2\,\%
		&
		
		23.4\,\%
		&
		9.1\,\%
		\\
	%	\midrule
		
		\hspace{-0.2cm}\parbox[t]{1cm}{\textsf{Practitioners}}
		%textsf{Practitioners}
		&
		49.5\,\%
		&
		55.9\,\%
		&
		51.6\,\%
		&
	
		21.5\,\%
		&
		11.8\,\%
		 \\
%		\midrule
		
		%\raisebox{-0\normalbaselineskip}[0pt][0pt]{\rotatebox[origin=c]{90}{\parbox{1.5cm}{textsf{Global\\ avoidance}}}}
		\hspace{-0.2cm}\parbox[t]{1cm}{\textsf{Academics}}
		%textsf{Academics}
		&
		67.9\,\%
		&
		51.8\,\%
		&
		30.4\,\%
		&
		
		26.8\,\%
		&
		3.6\,\%
		 \\
%		\midrule 
		
		%\raisebox{-0.2\normalbaselineskip}[0pt][0pt]{\rotatebox[origin=c]{90}{\parbox{1.5cm}{textsf{Future\\ avoidance}}}}	
		\hspace{-0.2cm}\parbox[t]{1cm}{\textsf{Leading roles}}
		%textsf{Leading roles}
		&
		41.7\,\%
		&
		56.2\,\%
		&
		56.2\,\%
		&
	
		20.8\,\%
		&
		10.4\,\%
		 \\
%		\midrule 
		
		%\raisebox{-0.9\normalbaselineskip}[0pt][0pt]{\rotatebox[origin=c]{90}{\parbox{1.7cm}{Up. Rest.\\ Avoidance}}}
		\hspace{-0.2cm}\parbox[t]{1cm}{\textsf{Programmers}}
		%textsf{Programmers}
		&
		57.8\,\%
		&
		55.6\,\%
		&
		46.7\,\%
		&
		22.2\,\%
		&
		13.3\,\%
		\\



		\bottomrule
	\end{tabular}
\end{table}


==> tables/open-source.tex <==

\begin{table}[b]
	\caption{Licensing models in used and released software: OS vs proprietary}
	\vspace{-0.2cm}
	\label{tab:license}
	\footnotesize
	\begin{tabular}{ p{1.5cm}  P{1.1cm} P{1.3cm} p{0.01cm} P{1.1cm} P{1.2cm}  } %{ l  c c c  c }
		\toprule
		& \multicolumn{2}{c }{\textsf{License of used libraries} } && \multicolumn{2}{c}{\textsf{License of own releases}}\\
		\cline{2-3}  \cline{5-6}
		& \textsf{OS}  & \textsf{proprietary} & & \textsf{OS} & \textsf{proprietary}\\
		\midrule 
		\hspace{-0.2cm}\parbox[t]{1cm}{\textsf{Overall}}	
		&
		97.4\,\%
		&
		43.5\,\%
		& &
		68.8\,\%
		&
		57.8\,\%
		\\
	%	\midrule
		
		\hspace{-0.2cm}\parbox[t]{1.2cm}{\textsf{Practitioners}}
		&
		96.8\,\%
		&
		47.3\,\%
		& &
		58.1\,\%
		&
		76.3\,\%
		 \\
%		\midrule
		
		%\raisebox{-0\normalbaselineskip}[0pt][0pt]{\rotatebox[origin=c]{90}{\parbox{1.5cm}{\emph{Global\\ avoidance}}}}
		\hspace{-0.2cm}\parbox[t]{1cm}{\textsf{Academics}}
		&
		98.2\,\%
		&
		37.5\,\%
		& &
		83.9\,\%
		&
		28.6\,\%
		 \\
%		\midrule 
		
		%\raisebox{-0.2\normalbaselineskip}[0pt][0pt]{\rotatebox[origin=c]{90}{\parbox{1.5cm}{\emph{Future\\ avoidance}}}}	
		\hspace{-0.2cm}\parbox[t]{1.7cm}{\textsf{Leading roles}}
		&
		97.9\,\%
		&
		54.2\,\%
		& &
		52.1\,\%
		&
		85.4\,\%
		 \\
%		\midrule 
		
		%\raisebox{-0.9\normalbaselineskip}[0pt][0pt]{\rotatebox[origin=c]{90}{\parbox{1.7cm}{Up. Rest.\\ Avoidance}}}
		\hspace{-0.2cm}\parbox[t]{1cm}{\textsf{Programmers}}
		&
		95.6\,\%
		&
		40\,\%
		& &
		64.4\,\%
		&
		66.7\,\%
		\\



		\bottomrule
	\end{tabular}
\end{table}


==> tables/participants.tex <==
\vspace{1cm}
\begin{table}
	\centering
	\begin{threeparttable}
		\caption{List of interviewees}
		\label{table:participants}
		
\begin{tabular}{l l l l l}

	&  \bfseries Case & \bfseries Role & \bfseries Exp. & \bfseries Exp. in Robotics\\
	\toprule
	1 & A & SM & 21 years & 6 years\\
	2 & B & CEO & 18 years & 18 years\\
	3 & C & SM &  11 years & 5 years\\
	4 & C & PM &  13 years & 6 years\\
	\midrule
	5 & D & SRSE & 15 years & 15 years\\
	6 & E & RE & 3 years & 2 years\\
	7 & F & SE &  13 years & 8 years\\
	8 & G & SD & 10 year & 5 years\\
	9 & H & RE & 2.5 years & 2.5 years\\
	10 & I & SE & 8 years & 6 years\\
	11 & C & TE & 19 years & 14 years\\
	12 & J & SAE & 8 years & 8 years\\
	13 & K & CEO & 15 years & 4 years\\
	14 & L & CEO & 11 year & 4 years\\
	15 & M & PM &  32 years & 21 years\\
	16 & N & PM &  11 years & 11 years\\
	17 & J & SAD &  11 years & 11 years\\
	18 & O & CTO &  8 years & 8 years\\
\bottomrule
	
\end{tabular}

%		\textbf{Case: } \patrizio{I don't think we can give these details now}
%		Company A (A) -> Conpleks (Sorin Adam);
%		Company B (B) -> BlueBotics (Nicola Tomatis);
%		Company C (C) -> Bosch (Mathias Buerger);
%		Company C (C) -> Bosch (Ralph Lange);
%		Company D (D) -> Eurecat (Davide Faconti);
%		Company E (E) -> PAL Robotics (Alessandro di Fava);
%		Company F (F) -> Robotnik (Roman Navarro);
%		Company G (G) -> PSB Intralogistics (Norbert Schmitz);
%		Company H (H) -> GMV (Guillermo Pati\~no);
%		Company I (I) -> PIAP Institute (Piotr Jaroszek);
%		Company C (C) -> Bosch (Ingo Lütkebohle);
%		Company J (J) -> Clearpath (Arron Griffiths);
%		Company K (K) -> Casual Robots (Pablo Medrano);
%		Company L (L) -> Aptomica (Per Sjoborg);
%		Company M (M) -> Dassault Aviation (Bruno Patin);
%		Company N (N) -> Fraunhofer IPA (Thilo Zimmermann);
%		Company J (J) -> Clearpath  (Enrique Fernandez);
%		Company O (O) -> Shape Robotics (Moises Pacheco);\\

%		\textbf{Case: } 
%		Company A (A);
%		Company B (B);
%		Company C (C);
%		Company C (C);
%		Company D (D);
%		Company E (E);
%		Company F (F);
%		Company G (G);
%		Company H (H);
%		Company I (I);
%		Company C (C);
%		Company J (J);
%		Company K (K);
%		Company L (L);
%		Company M (M;
%		Company N (N);
%		Company J (J);
%		Company O (O);\\
		\textbf{Roles:} System Manager (SM);
			Chief Executive Officer (CEO);
			Senior Manager (SM); 
			Project Manager (PM);
			Senior Robotic Software Engineer (SRSE);
			Robotics Engineer (RE);
			Software Engineer (SE);
			Software Developer (SD);
			Technical Expert (TE);
			Senior Application Engineer (SAE);
			Senior Autonomy Developer (SAD);
			Chief Technology Officer (CTO).
	\end{threeparttable}
\end{table}

==> tables/service.tex <==

\begin{table}[h!]
	\small
	\caption{Provided service or product}
	\vspace{-0.2cm}
	\label{tab:service}
	\begin{tabular}{ p{1.5cm}  P{1.45cm} P{1.1cm} P{0.9cm} P{0.9cm} P{0.5cm} }
		\toprule
		& \textsf{Low-level}  & \textsf{Planning} & \textsf{Complete} & \textsf{Drivers} & \textsf{Other}\\
		& \textsf{functionalities}  & \textsf{modules} & \textsf{System} & &\\
		\midrule 
		\hspace{-0.2cm}\parbox[t]{1cm}{\textsf{Overall}}	
		&
		66.4\,\%
		&
		63.6\,\%
		&
		51.3\,\%
		&
		44.8\,\%
		&
		9.1\,\%
		\\

		
		\hspace{-0.2cm}\parbox[t]{1.2cm}{\textsf{Practitioners}}
		&
		60.2\,\%
		&
		58.1\,\%
		& 
		59.1\,\%
		&
		45.2\,\%
		&
		9.7\,\%
		 \\

		

		\hspace{-0.2cm}\parbox[t]{1cm}{\textsf{Academics}}
		&
		73.2\,\%
		&
		75\,\%
		& 
		39.3\,\%
		&
		44.6\,\%
		&
		8.9\,\%
		 \\

		

		\hspace{-0.2cm}\parbox[t]{1.6cm}{\textsf{Leading roles}}
		&
		64.6\,\%
		&
		68.8\,\%
		& 
		54.2\,\%
		&
		50\,\%
		&
		8.3\,\%
		 \\

		

		\hspace{-0.2cm}\parbox[t]{1cm}{\textsf{Programmers}}
		&
		55.6\,\%
		&
		46.7\,\%
		&
		 64.4\,\%
		 &
		40\,\%
		&
		11.1\,\%
		\\



		\bottomrule
	\end{tabular}
\end{table}

